Provable Routing Analysis of Programmable Photonics

Programmable photonic integrated circuits (PPICs) are an emerging technology recently proposed as an alternative to custom-designed application-specific integrated photonics. Light routing is one of the most important functions that need to be realized on a PPIC. Previous literature has investigated the light routing problem from an algorithmic or experimental perspective, e.g., adopting graph theory to route an optical signal. In this paper, we also focus on the light routing problem, but from a complementary and theoretical perspective, to answer questions about what is possible to be routed. Specifically, we demonstrate that not all path lengths (defined as the number of tunable basic units that an optical signal traverses) can be realized on a square-mesh PPIC, and a rigorous realizability condition is proposed and proved. We further consider multi-path routing, where we provide an analytical expression on path length sum, upper bounds on path length mean/variance, and the maximum number of realizable paths. All of our conclusions are proven mathematically. Illustrative potential optical applications using our observations are also presented.

==> dummy.tex <==

To begin with, Fig.~\ref{fig:splitting_tree} (b) demonstrates how to achieve $1$-to-$4$ splitting using a $4\times 3$ square mesh. It utilizes the construction for $1$-to-$2$ splitting shown in Fig.~\ref{fig:splitting_tree} (a). Namely, we first do a vertical flipping (marked by the blue arrow) of the schematic shown in (a) \footnote{It is not a strict vertical flipping, as we will keep the phase shift configuration in the first column unchanged. Namely, $\pi$ is on the upper arm and $0\pi$ on the lower arm.}, and then connect these two sub-parts with an additional splitting structure (marked by black), which is made available by an additional column (marked by pink) in (b). With some calculations, we could show that the complex magnitude at node N2 and N4 are both $(0.5-0.5\cj)^2\e^{-\cj 6\omega n_{\text{eff}}L/c}$. The responses at node N1 and N3 are identical, and compared to node N2 and N4, they have an additional $\pi$ phase shift as evident by the second line in Eq.~(\ref{eq:cross_bar}). This approach could be generalized to any $1$-to-$2^d$ splitting (where $d$ is an positive integer). Specifically, to implement $1$-to-$2^d$ splitting, we need a $2^d$-by-$(d+1)$ square mesh, and the responses at the $2^{d-1}$ nodes \{N2, N4, $\cdots$, N$2^d$\} are identical. Fig.~\ref{fig:splitting_tree} (a) and (b) respectively demonstrate the case of $d=1$ and $d=2$. 

% In silicon photonics, beam steering is usually realized by an application-specific circuit, such as an optical phased shift array (OPA)~\cite{kim2019opa}. A conventional OPA consists of a splitting tree, an array of tunable phase shifts and antennas~\cite{kim2019opa}. Note that we are not advocating square-mesh PPIC over an OPA when doing beam steering, but rather exhibit that the PPIC, a generic circuit, also has the ability to achieve the goal.



\begin{figure}[!htb]
    \centering
    \includegraphics[width=1.0\linewidth]{figs/splitting_tree.png}
    \caption{(a) Top row: construction for $1$-to-$2$ splitting in a $2\times 2$ square mesh. Bottom row: when injecting an optical signal with complex magnitude equal to $(1+0\cj)$, the complex magnitudes of the output signals are shown. The dependence on $\alpha \e^{-\cj\omega n_{\text{eff}}L/c}$ is not included for clearness. As an example, the complex magnitude of the output signal at node N2 is actually $(0.5-0.5\cj)\e^{-\cj 4\omega n_{\text{eff}}L/c}$. (b) Construction for $1$-to-$4$ splitting in a $4\times 3$ square mesh. The complex magnitude at node N2 and N4 are both $(0.5-0.5\cj)^2\e^{-\cj 6\omega n_{\text{eff}}L/c}$.}
    \label{fig:splitting_tree}
\end{figure}



In short, our construction provides a way to do $1$-to-$2^d$ splitting. To complete the task of beam steering, we also need an optical delay line network. We could do so by appending a $2^d$-by-$2^d$ square mesh to the left side of the splitting tree network demonstrate in Fig.~\ref{fig:splitting_tree} (b). Taking $d=2$ as an example, if we append the network shown in Fig.~\ref{fig:optical_delay_line_network} to the left side of Fig.~\ref{fig:splitting_tree} (b), then the magnitude at port P4 and P2 will have a phase difference equal $4\omega n_{\textbf{eff}}L/c$. If we further connect optical antenna at port P2 and P4, we obtain a linear antenna array with two elements~\cite{kim2019opa}. Note that the port P1 and P3 corresponding to node N1 and N3 could be used to implement another linear antenna array.

In summary, to realize a linear antenna array with $2^{d-1}$ elements, we need an overall $2^d$-by-$(2^d+d+1)$ square mesh, where the last $(d+1)$ columns are used to realize a splitting tree, and the first $2^d$ columns for optical delay lines. When injecting a source of $(1+0\cj)$ as demonstrate in Fig.~\ref{fig:splitting_tree} (b) from the right side, the resulting port responses at \{P1,P2,$\cdots$, P$2^{d-1}$\} have same magnitude, and they have a phase slope equal to $4\omega n_{\text{eff}}L/c$. Furthermore, the steering angle $\gamma$ is known related to the phase slope:
\begin{equation}\label{eq:true_time_delay}
    \sin\gamma=\frac{\text{phase slope}}{kd}=\frac{4(\omega n_{\text{eff}}L/c+\epsilon)}{kd}=\frac{4n_{\text{eff}}L}{d}+\frac{2\epsilon\lambda}{\pi d}
\end{equation}
where $d$ represents the spacing between antenna elements. Eq.~(\ref{eq:true_time_delay}) indicates that this constructed antenna array using square mesh actually uses the concept of true time-delay beam steering~\cite{Longbrake2012true}. It has the benefit of small beam squint among a certain frequency range. Namely, when adjusting the wave frequency, if $n_{\text{eff}}$ doesn't change much along frequency, then the steering angle won't change . Furthermore, notice that we have tremendous redundant phase shifts in the square mesh, wich 


\begin{figure}
    \centering
    \includegraphics[width=1.0\linewidth]{figs/optical_delay_line.png}
    \caption{Optical delay line network. The final optical signal response at port P2 is $(0.5-0.5\cj)^2\e^{-\cj 10\omega n_{\text{eff}}L/c}$, and that at port P4 is $(0.5-0.5\cj)^2\e^{-\cj 14\omega n_{\text{eff}}L/c}$. }
    \label{fig:optical_delay_line_network}
\end{figure}

